Randomness in large language models: What researchers need to know (and report)

Large language models (LLMs) are increasingly used to generate data for research. Typical use cases are classifications, annotations, information extraction, and generation of numerical scores. Unlike conventional measurements, LLM outputs can vary across repeated requests even when the prompt and apparent model settings remain unchanged. This variation arises from deliberate sampling, silent model updates, numerical rounding, or expert routing. Setting a dedicated temperature parameter to zero removes deliberate sampling when that option is available, but it does not eliminate the other sources of randomness. Exact reproduction is therefore generally not possible when using proprietary application programming interfaces. Local execution of open-weight models offers greater control, but reproducibility still depends on the complete hardware and software stack. We illustrate these issues through sentiment classifications of corporate filings and examine their consequences for downstream regression results. We then propose a reporting standard for articles and replication packages, as well as guidance for data editors and authors. Together, these findings and recommendations establish that LLM outputs should be treated as draws from a distribution rather than as fixed measurements.

==> tables/hardware_audit.tex <==
% Auto-generated by scripts/hardware_audit_table.py -- do not edit by hand.
\begin{tabular}{@{}L{0.32\textwidth}L{0.58\textwidth}@{}}
\toprule
Check & Result \\
\midrule
Input filings (NSC.txt, VRSN.txt) & Identical: both runs at commit 3ee413f, where the excerpts are tracked; identical to the shipped excerpts \\
Yahoo returns data & Consistent: all 800 recorded regressions of both runs reproduce from the shipped returns (largest coefficient difference $1\times 10^{-7}$, Yahoo's float rounding) \\
Model weights/revision & Identical (6b06e97d84a3) \\
Software & Identical: mlx 0.32.4, mlx-vlm 0.7.12, transformers 5.22.2 \\
Firm count, $T{=}0$ row count & Identical: 100 firms, 20{,}000 rows each \\
Internal consistency (200 runs/firm at $T{=}0$) & Perfect: each firm's output is 100\% stable across all 200 runs on a given machine \\
Actual divergence & Exactly 2 firms, NSC and VRSN (NSC: neutral on the M1 Pro, negative on the M4; VRSN: negative on the M1 Pro, neutral on the M4), each consistent across all runs \\
\bottomrule
\end{tabular}


==> tables/hardware_label_instability.tex <==
% Auto-generated by scripts/hardware_summary_tables.py -- do not edit by hand.
\begin{tabular}{lcccccc}
\toprule
Machine & $K$ ($T{=}0$) & $k$ ($T{=}0$) & Agreement \% ($T{=}0$) & $K$ ($T{=}1.5$) & $k$ ($T{=}1.5$) & Agreement \% ($T{=}1.5$) \\
\midrule
PTL11077 (M1 Pro) --- reference & 0 & 0.0 & 100.0 & 25 & 1.69 & 97.7 \\
PCPEM52119 (M4) & 0 & 0.0 & 100.0 & 31 & 0.99 & 98.3 \\
il-lv39 (M4 Max) & 0 & 0.0 & 100.0 & 31 & 0.96 & 98.3 \\
cbsugpu06 (A40) & 0 & 0.0 & 100.0 & 54 & 1.31 & 97.8 \\
cv-ai (RTX 3060 $\times$2) & 0 & 0.0 & 100.0 & 52 & 1.48 & 97.7 \\
cbsugpu06 (A40 $\times$2) & 0 & 0.0 & 100.0 & 54 & 1.31 & 97.8 \\
cbsugpu10 (RTX 6000 Ada) & 0 & 0.0 & 100.0 & 58 & 1.47 & 97.6 \\
cv-ai (RTX 3060 $\times$2, re-run) & 0 & 0.0 & 100.0 & 52 & 1.48 & 97.7 \\
\bottomrule
\end{tabular}


==> tables/hardware_results.tex <==
% Auto-generated by scripts/hardware_summary_tables.py -- do not edit by hand.
\begin{tabular}{llcc}
\toprule
Hardware & Backend & $T{=}0$ coefficient (SD) & $T{=}1.5$ mean coefficient (SD) \\
\midrule
PTL11077 (M1 Pro) --- reference & MLX & $-0.1224$ (0) & $-0.1245$ (0.0261) \\
PCPEM52119 (M4) & MLX & $-0.1386$ (0) & $-0.1335$ (0.0351) \\
il-lv39 (M4 Max) & MLX & $-0.1386$ (0) & $-0.1361$ (0.0315) \\
cbsugpu06 (A40) & CUDA & $-0.0718$ (0) & $-0.1038$ (0.1133) \\
cv-ai (RTX 3060 $\times$2) & CUDA & \multicolumn{1}{c}{$^{a}$} & $-0.0505$ (0.1288) \\
cbsugpu06 (A40 $\times$2, split) & CUDA & $-0.0718$ (0)$^{b}$ & $-0.1038$ (0.1133) \\
cbsugpu10 (RTX 6000 Ada) & CUDA & $-0.0718$ (0) & $-0.0878$ (0.0999) \\
cv-ai (RTX 3060 $\times$2, re-run) & CUDA & \multicolumn{1}{c}{$^{a}$} & $-0.0505$ (0.1288) \\
\bottomrule
\end{tabular}


==> tables/hardware_variance_diagnostics.tex <==
% Auto-generated by scripts/hardware_summary_tables.py -- do not edit by hand.
\begin{tabular}{lcc}
\toprule
Machine & SD(coef)/mean SE, $T{=}0$ & SD(coef)/mean SE, $T{=}1.5$ \\
\midrule
PTL11077 (M1 Pro) --- reference & $<0.001$ & 0.183 \\
PCPEM52119 (M4) & $<0.001$ & 0.247 \\
il-lv39 (M4 Max) & $<0.001$ & 0.222 \\
cbsugpu06 (A40) & $<0.001$ & 0.486 \\
cv-ai (RTX 3060 $\times$2) & ---$^{a}$ & 0.550 \\
cbsugpu06 (A40 $\times$2) & $<0.001$ & 0.486 \\
cbsugpu10 (RTX 6000 Ada) & $<0.001$ & 0.424 \\
cv-ai (RTX 3060 $\times$2, re-run) & ---$^{a}$ & 0.550 \\
\bottomrule
\end{tabular}


==> tables/variance_diagnostics.tex <==
% Auto-generated by scripts/build_variance_diagnostics_table.py -- do not edit by hand.
% Source: data/crosscheck/{variance_diagnostics,label_instability,deepseek_temp0_distinct_values}.csv
% Referee comment #8 (R1), gh issue #10 (subs #11-#13).
\begin{table}[h]
\centering
\caption{Variance and label-instability diagnostics across repeated runs, by model.}
\label{tab:r1comment8}
\small
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{SD(coef) / mean within-run SE} & \multicolumn{2}{c}{Firms ever flip label (/100)} & \multicolumn{2}{c}{Pairwise run agreement (\%)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Model & $T{=}0$ & $T{>}0$ & $T{=}0$ & $T{>}0$ & $T{=}0$ & $T{>}0$ \\
\midrule
DeepSeek-v4-pro$^{a}$ & 0.26 & 0.69 & 2 & 69 & 99.7 & 95.4 \\
GPT-5.6-luna$^{b}$ & -- & 0.69 & -- & 71 & -- & 82.9 \\
Gemma-4-26b$^{c}$ & $<0.001$ & 0.18 & 0 & 25 & 100.0 & 97.7 \\
\bottomrule
\end{tabular}
\par\smallskip
\footnotesize
$^a$DeepSeek's $T{>}0$ column is the API default (temperature omitted). $\quad$
$^b$GPT-5.6 has no $T{=}0$ leg (no explicit temperature control); its one condition is shown under $T{>}0$. $\quad$
$^c$Gemma's $T{>}0$ column is $T{=}1.5$; its $T{=}0$ leg is internally deterministic.

\smallskip
\noindent DeepSeek's 200 ``identical'' $T=0$ runs collapse to 4 distinct (coefficient, $t$-statistic) pairs: $(-0.279,\,-1.79)$ in 20 runs, $(-0.192,\,-1.42)$ in 168 runs, $(-0.158,\,-0.82)$ in 2 runs, $(-0.085,\,-0.55)$ in 10 runs -- a range of 0.19 in the coefficient and 1.24 in the $t$-statistic, traced to the 2 firms (of 100) whose label flips at $T=0$.
\end{table}

